QEBA: Query-Efficient Boundary-Based Blackbox Attack

Machine learning (ML), especially deep neural networks (DNNs) have been widely used in various applications, including several safety-critical ones (e.g. autonomous driving). As a result, recent research about adversarial examples has raised great concerns. Such adversarial attacks can be achieved by adding a small magnitude of perturbation to the input to mislead model prediction. While several whitebox attacks have demonstrated their effectiveness, which assume that the attackers have full access to the machine learning models; blackbox attacks are more realistic in practice. In this paper, we propose a Query-Efficient Boundary-based blackbox Attack (QEBA) based only on model's final prediction labels. We theoretically show why previous boundary-based attack with gradient estimation on the whole gradient space is not efficient in terms of query numbers, and provide optimality analysis for our dimension reduction-based gradient estimation. On the other hand, we conducted extensive experiments on ImageNet and CelebA datasets to evaluate QEBA. We show that compared with the state-of-the-art blackbox attacks, QEBA is able to use a smaller number of queries to achieve a lower magnitude of perturbation with 100% attack success rate. We also show case studies of attacks on real-world APIs including MEGVII Face++ and Microsoft Azure.

==> backup.tex <==
\subsection{Why Direct Gradient Estimation is Inefficient}
% Eqn.\ref{eqn:grad-est} provides a way to estimate gradients via decision-based black-box access to the model. However, this estimation may not be accurate enough by noticing that $\widetilde{\nabla S}$ is a linear combination of $B$ vectors in $\mathbb{R}^m$. In practice, $m$ may be very large (e.g. $3\times224\times224$ in most pretrained models on ImageNet) while $B$ is chosen to be small (e.g. 100). Therefore, even in the best case the approximation is only the projection of the gradient $\nabla S$ onto the subspace spanned by $u_1,\ldots,u_B$. Considering that $u$'s are randomly chosen, the approximation may not be good. In particular, we have the following theorem on the expected quality of the estimated gradient:
The gradient vector estimated by Eqn. \ref{eqn:grad-est} is a linear combination of $B$ vectors $u_1,\ldots,u_B \in \mathbb{R}^m$.  The best estimated gradient we can possibly get is the projection of the actual gradient onto the subspace spanned by the $B$ vectors. In practice, $m$ is large (for example, $3\times224\times224$ on ImageNet) while $B$ is chosen to be small (e.g., 100). The following theorem shows the expectation of the gradient approximation in a randomly sampled subspace. 
\begin{theorem}
\label{tho:cos}
For a boundary point $x$, suppose that $S(x)$ has $L$-Lipschitz gradients in a neighborhood of $x$, and that the sampled ${\bf u}_1, \ldots, {\bf u}_B$ are orthogonal to each other. Then the expected cosine simliarity between $\widetilde{\nabla S}$ and $\nabla S$ can be bounded by:
\begin{align}
    & \bigg( 2\bigg(1-(\frac{L\delta}{2||\nabla S||_2})^2\bigg)^{\frac{m-1}{2}} - 1 \bigg)c_m\sqrt{\frac B m}\\
    \leq & \mathbb{E}\big[\cos (\widetilde{\nabla S}, \nabla S) \big]\\
    \leq & c_m\sqrt{\frac B m}
\end{align}
% \begin{align}
%     \bigg( 2\bigg(1-(\frac{L\delta}{2||\nabla S||_2})^2\bigg)^{\frac{m-1}{2}} - 1 \bigg)c_m\sqrt{\frac B m}
%     & \leq \mathbb{E}\big[\cos (\widetilde{\nabla S}, \nabla S) \big]\\
%     \mathbb{E}\big[\cos (\widetilde{\nabla S}, \nabla S) \big] &\leq c_m\sqrt{\frac B m}
% \end{align}
where $c_m$ is a constant related with $m$ and can be bounded by $c_m \in (2/\pi, 1)$. In particular, we have:
\begin{align}
    \label{eqn:grad-est-qual}
    \lim_{\delta\rightarrow 0}\mathbb{E}\big[\cos (\widetilde{\nabla S}, \nabla S) \big] = c_m\sqrt{\frac B m}.
\end{align}
\end{theorem}
The proof of Theorem \ref{tho:cos} is in Appendix \ref{sec:proof}. We see that in the case of $m=3\times224\times224$ and $B=100$, the expected cosine similarity between the estimation and the ground truth gradient is only around 0.02.
Hence, we claim that direct gradient estimation, i.e. estimating by sampling directly from the entire space, cannot achieve a good gradient estimation.
% , which means we can estimate only a small portion of the gradient direction.
% Our observation in the experiments\Xiaojun{add if we have space} matches this conclusion.
% Hence, we may expect better attack performance if we can produce better gradient estimation using the same number of queries.
This also suggests that a better approximation can be expected if we can estimate the gradient in a lower-dimensional space. \Huichen{I think the logic in the writing here is a little bit weird, but I don't know how to improve it..}
